Local Correlation Clustering with Asymmetric Classification Errors

In the Correlation Clustering problem, we are given a complete weighted graph $G$ with its edges labeled as "similar" and "dissimilar" by a noisy binary classifier. For a clustering $\mathcal{C}$ of graph $G$, a similar edge is in disagreement with $\mathcal{C}$, if its endpoints belong to distinct clusters; and a dissimilar edge is in disagreement with $\mathcal{C}$ if its endpoints belong to the same cluster. The disagreements vector, $\text{dis}$, is a vector indexed by the vertices of $G$ such that the $v$-th coordinate $\text{dis}_v$ equals the weight of all disagreeing edges incident on $v$. The goal is to produce a clustering that minimizes the $\ell_p$ norm of the disagreements vector for $p\geq 1$. We study the $\ell_p$ objective in Correlation Clustering under the following assumption: Every similar edge has weight in the range of $[\alpha\mathbf{w},\mathbf{w}]$ and every dissimilar edge has weight at least $\alpha\mathbf{w}$ (where $\alpha \leq 1$ and $\mathbf{w}>0$ is a scaling parameter). We give an $O\left((\frac{1}{\alpha})^{\frac{1}{2}-\frac{1}{2p}}\cdot \log\frac{1}{\alpha}\right)$ approximation algorithm for this problem. Furthermore, we show an almost matching convex programming integrality gap.

==> figures/image_intGap.tex <==

% In this section, we present an integrality gap example for the convex program $(P)$ in Figure~\ref{fig:CP}. 
% We consider a special case of Corrleation Clustering with Asymmetric Classification Errors: $s-t$ cut with Asymmetric Classification Errors. Our integrality gap instance consisits of a layered graph and is motivated by [NIPS 2019]. For a fixed $\alpha > 0$, we consider a graph on $n$ vertices, where $n$ is parameterized by $\alpha$. Specifically, the instance consists of abput $poly(\frac{1}{\alpha})$ layers which are heavily inter-connected. Thus, any integral solution separating $s$ and $t$ must disconnect at least one pair of consecutive layers and thus any vertex in these layers will be incident to a lot of cut edges. While the LP solution can ``average'' the cut across multiple layers which ensures that no particular vertex in any layer incurs a heavy cut. We note that as the graphs is complete, any solution (integral or fractional) has to cut a lot of ``intra'' layer edges. By ensuring that the edges connecting consecutive layers cost significantly more, we can penalize the integral solution more heavily. 

% We will show the following theorem, 

% \begin{theorem}
% The integrality gap for the convex relaxation $(P)$ (\ref{fig:CP}) has an integrality
% gap of $\Omega\bigg((\frac{1}{\alpha})^{\frac{1}{2} - \frac{1}{2q}}\bigg)$ for the $\ell_p$ objective in the $s-t$ cut with Asymmetric Classification Errors model.
% \end{theorem}

% \begin{proof}
% We now describe our construction in detail. The graph $G$ consists of $m$ layers of $k$ nodes each. Let $l_i$ denote the $i$-th layer. For each $i \in \{1, 2, \ldots, m-1\}$, layer $l_i$ is completely connected to layer $l_{i+1}$ using edges of weight $1$. In addition to these $k \cdot m$ nodes, we have two nodes $s$ and $t$. 
% We connect $s$ to $l_1$ via a complete graph on $k_n$ nodes - we connect $s$ to all the $n$ vertices in $K_n$ using edges of weight $1$ each and then all the vertices of $K_n$ to layer $l_1$ using edges of weight $1$ each. We similarly connect $t$ to $l_m$ via another complete graph $K_n$. 
% %We want to connect $s$ and $t$ to $l_1$ and $l_m$ and at the same time ensure that none of these edges are part of the integral solution. We can do this by connecting $s$ to all the verties of the complete graph $K_n$, and then connecting all the vertices of the $k_n$ to layer $l_1$. We will similarly connect $t$ to $l_m$.
% Let $E_1$ be the set of all edges (of weight $1$). The graph is made complete, using edges of weight $\alpha$. That is, $E_\alpha = (V \times V) \setminus E_1$.

% Now, consider any integral cut separating $s$ and $t$ in the graph. 
% Any such cut cannot separate $s$ from $l_1$ or $t$ from $l_m$ without incurring a heavy penalty on $s$ or $t$. Thus, any such cut should separate $l_i$ from $l_{i+1}$ for some $i \in \{1, 2, \ldots, m-1\}$. Otherwise, if all consecutive layers are connected, it means that there exists a path from $s$ to $t$. Thus assume that there is an integral cut that separates $l_j$ from $l_{j+1}$ for some $j \in \{1, 2, \ldots, m-1\}$. For each vertex $u$ in layer $l_j$ and $l_{j+1}$, $u$ has $k$ edges of weight $1$ that are cut. In addition, the edges of weight $\alpha$ incident to $u$ that are cut are at most $n$. Thus $OPT^q = \Omega(k \cdot (k + \alpha n)^q)$.

% Now, consider the following fractional cut separating $s$ and $t$. Let $E_l$ be the set of edges that are present between consecutive layers. That is, $E_l = \{(u,v): $u \in l_i$\text{ and }$v \in L_{i+1}\text{ for some }$i \in [m]\}$. Each edge $(u,v) \in E_l$ is assigned the value $x_{uv} = \frac{1}{m}$. We then compute the shortest path metric using the edges $E_l$ to assign a fractional weight to all the edges.
% That is, for any other edge $(u',v') \in E$, we assign $x_{u'v'}$ to be the shortest distance between $u'$ and $v'$ using the edges $E_l$.
% Finally, the weight of the cut at any vertex $u$ is $(\frac{k}{m} + \alpha n)$. 

% Thus, 

% $$OPT^q = k(k + \alpha n)^q \approx k^{q+1}$$

% $$LP^q = km (\frac{k}{m} + \alpha n)^q$$

% Setting $\frac{k}{m} = \alpha n$, we get $m = \Omega(\frac{1}{\sqrt{\alpha}})$ and, 

% $$\frac{OPT^q}{LP^q} = k^{q+1}/ \frac{k^{q+1}}{m^{q-1}} = m^{q-1} = (\frac{1}{\sqrt{\alpha}})^{q-1}$$

% Thus, $\frac{OPT}{LP} = \Omega\bigg((\frac{1}{\alpha})^{\frac{1}{2} 


\begin{center}
\begin{tikzpicture}
%Layer 1
\fill[fill=black!20!white,draw=black,thick] (-13,0) ellipse (1 and 3.3);
\node[shape=circle,fill=black] (j1) at (-13,2.5) {};
\node[shape=circle,fill=black] (j2) at (-13,2) {};
\node[shape=circle,fill=black] (j3) at (-13,-2.5) {};

\path (j2) -- (j3) node [black, font=\Huge, midway, sloped] {$\dots$};

%Layer 2
\fill[fill=black!20!white,draw=black,thick] (-10,0) ellipse (1 and 3.3);
\node[shape=circle,fill=black] (m1) at (-10,2.5) {};
\node[shape=circle,fill=black] (m2) at (-10,2) {};
\node[shape=circle,fill=black] (m3) at (-10,-2.5) {};
\path (m2) -- (m3) node [black, font=\Huge, midway, sloped] {$\dots$};

%Layer 3
\fill[fill=black!20!white,draw=black,thick] (-7,0) ellipse (1 and 3.3);
\node[shape=circle,fill=black] (k1) at (-7,2.5) {};
\node[shape=circle,fill=black] (k2) at (-7,2) {};
\node[shape=circle,fill=black] (k3) at (-7,-2.5) {};

\path (k2) -- (k3) node [black, font=\Huge, midway, sloped] {$\dots$};


\node at (-5,0) {$\dotsb$};

%Layer 4
\fill[fill=black!20!white,draw=black,thick] (-2.5,0) ellipse (1 and 3.3);
\node[shape=circle,fill=black] (l1) at (-2.5,2.5) {};
\node[shape=circle,fill=black] (l2) at (-2.5,2) {};
\node[shape=circle,fill=black] (l3) at (-2.5,-2.5) {};


\path (l2) -- (l3) node [black, font=\Huge, midway, sloped] {$\dots$};

\node[shape=circle, fill=white, draw=black] (s) at (-16,0) {$s$};
\node[shape=circle, fill=white, draw=black] (t) at (1,0) {$t$};

\draw[draw=red]  (s) edge node {} (j1);
\draw[draw=red]  (s) edge node {} (j2);
\draw[draw=red]  (s) edge node {} (j3);

\draw[draw=red]  (t) edge node {} (l1);
\draw[draw=red]  (t) edge node {} (l2);
\draw[draw=red]  (t) edge node {} (l3);

%edges between layer 2 and 3
\draw[draw=black]  (m1) edge node {} (k1);
\draw[draw=black]  (m1) edge node {} (k2);
\draw[draw=black]  (m1) edge node {} (k3);

\draw[draw=black]  (m2) edge node {} (k1);
\draw[draw=black]  (m2) edge node {} (k2);
\draw[draw=black]  (m2) edge node {} (k3);

\draw[draw=black]  (m3) edge node {} (k1);
\draw[draw=black]  (m3) edge node {} (k2);
\draw[draw=black]  (m3) edge node {} (k3);

%edges between layer 1 and 2
\draw[draw=black]  (m1) edge node {} (j1);
\draw[draw=black]  (m1) edge node {} (j2);
\draw[draw=black]  (m1) edge node {} (j3);

\draw[draw=black]  (m2) edge node {} (j1);
\draw[draw=black]  (m2) edge node {} (j2);
\draw[draw=black]  (m2) edge node {} (j3);

\draw[draw=black]  (m3) edge node {} (j1);
\draw[draw=black]  (m3) edge node {} (j2);
\draw[draw=black]  (m3) edge node {} (j3);


\draw [decorate,decoration={brace,amplitude=10pt},xshift=0.8cm,yshift=0pt]
(-6.9,3) -- (-6.9,-3) node [black,midway,xshift=0.55cm]
{\footnotesize $k$};

\draw [decorate,decoration={brace,amplitude=10pt},xshift=0cm,yshift=0.45pt]
(-13.5,3.5) -- (-2,3.5) node [black,midway,yshift=0.55cm]
{\footnotesize $m$};

\end{tikzpicture}
\end{center} 


==> paper/decomposition.tex <==
\section{Probabilistic Metric Space Decomposition}\label{sec:decomposition}

\knote{We should probably mention Padded Decomposition and compare this decomposition with the padded decomposition (just 1-2 paragraphs.}
\knote{Also, need to quote some papers on the padded/separating decomposition}
\snote{I will pick up the token on this}
\begin{theorem}\label{thm: decompositon}
Consider a finite metric space $(X,d)$. Fix two positive numbers $r$ and $R$ with $r<R$. Let $\beta = r/R$ and $q\geq 1$. Then, there exists a probabilistic partitioning $\calP$ and function $D_{\beta}=O(q\log\nicefrac{1}{\beta})$ satisfying the following properties:

%\begin{enumerate}[label=(\alph*)]
\noindent (a) 
%\item 
    $\diam(P)\leq 2R$ for every $P\in \calP$ (always);  

%%    
%%\item
\noindent (b) For every point $u$ in $X$, the following bound holds:
    \begin{multline*}
    \sum_{v\in \ball(u,R)}\Bigg(\Pr\big\{\calP(u)\neq \calP(v)\big\} - 
    D_{\beta}\frac{d(u,v)}{R}\Bigg)^+
    \lesssim\\
    \lesssim
    \beta^q
    \sum_{v\in \ball(u,2R)} \frac{d(u,v)}{R}.       
    \end{multline*}
%%    
%%\item
\noindent (c) Moreover, for every $u$ in $X$, we always have, 
    \begin{multline*}
    \sum_{v\in \ball(u,r)}\one\big\{\calP(u)\neq \calP(v)\big\}\lesssim\\ \lesssim
    \beta \cdot D^2_{\beta}
    \sum_{v\in\ball(u,2R)}\frac{d(u,v)}{R}.
    \end{multline*}
%%\end{enumerate}
\end{theorem}



\input{figures/algo_MPSP}

==> paper/item-b-lemma.tex <==
\section{Proof of Lemma~\ref{lem:item-b-helper}}\label{sec:lem:item-b-helper}
\begin{proof}[Proof of Lemma~\ref{lem:item-b-helper}]
Consider one term from the left hand side of condition~(b) of Theorem~\ref{thm:itr-clustering}:
$$
\Big(\Pr\big\{\delta_P(u,v) =1 \big\} 
- D_{\beta}\frac{d(u,v)}{R} \cdot \Pr\{\vee_P(u,v)=1\}\Big)^+.
$$
Note that $\{\delta_P(u,v) = 1\}$ denotes the event that \textit{exactly one of the points} $u$ \textit{and} $v$ lies in $P$;
whereas $\{\vee_P(u,v) = 1\}$ denotes the event that \textit{at least} one of $u$ or $v$
lies in $P$. Thus, $\Pr\{\vee_P(u,v) = 1\} \geq \Pr\{\delta_P(u,v) = 1\}$. Hence, this expression is positive only if $D_{\beta}\cdot d(u,v)/R < 1$, which is equivalent to
$$d(u,v) < R/D_{\beta} = R_0.$$
Thus, in the left hand side of condition (b), we can consider only $v$ in $\ball(u,R_0)$ 
(rather than $\ball(u,R)$). Moreover, if $d(z,u)> R$, then for all $v \in \ball(u,R_0)$, we have $d(z,v) > R-R_0$ and, consequently, $\delta_P(u,v)=0$. Therefore, for such $u$, the left hand side of condition (b) equals $0$, and the inequality (b) holds trivially. We will thus assume that $d(z,u)\leq R$. Similarly, since $t > 3R_0$, we will assume that $d(z,u)\geq 2R_0$ (otherwise, $u\in P$ and every $v\in \ball(u,R_0)$ is in $P$, and thus $\delta_P(u,v) = 0$).

We now show that if Condition I or II of~Lemma~\ref{lem:item-b-helper} holds that (b) is satisfied. 

I. Suppose, the first condition holds for $u\in \ball(z,R)$. If $\delta_P(u,v) = 0$. then either $u\in P$ or $v\in P$. In the former case, $t\geq d(z,u)$; in the latter case, $t\geq d(z,v) \geq d(z, u) - R_0$. In either case, $t\geq d(z, u) - R_0$.
Using that $|\ball(u, R_0)| \leq |\ball(z, R_0)|$ by our choice of $z$ (see (\ref{pvt-condition})), we bound the left hand side of (b) as follows
\begin{align*}
\sum_{v\in \ball(u, R_0)}&\Pr\{\delta_P(u,v)=1\}
\\ &\leq 
|\ball(u, R_0)|\Pr\{t \geq d(z,u)-R_0\}
\\ &\leq 
|\ball(z, R_0)|\Pr\{t \geq d(z,u)-R_0\}
\end{align*}
%Here, we used that $d(z,v)\geq d(z,u)-R_0$. Thus, if 
%$\delta_P(u,v)=1$, then we must have $t \geq d(z,u)-R_0$.
We now use the inequality from Condition I to get the bound
\begin{align*}
\sum_{v\in \ball(u, R_0)}\Pr\{\delta_P(u,v)=1\}&
\lesssim \beta^{q+1} \E|\ball(z,t)|\\
&=\beta^{q+1}\E|P|.    
\end{align*}
Finally, by Lemma~\ref{lem:item-Y-helper}, we have the following bound for the right hand side of (b):
\begin{equation}\label{eq:beta-Y-P}
\beta^q\E[Y_t]\geq \beta^{q} D_{\beta}^{-1}\E|P|/2
\gtrsim \beta^{q+1} \E|P|.
\end{equation}

\noindent II. Suppose now that the second condition holds for $u\in \ball(z,R)$. Then, each term in the left hand side of (b) is upper bounded by $O(\beta^{q+1})$. Hence, the entire sum is upper bounded by $O(\beta^{q+1}|\ball(u,R_0)|)$, which in turn is upper bounded by $O(\beta^{q+1}|\ball(z,R_0)|)$. We now lower bound the right hand side of (b) using Inequality~(\ref{eq:beta-Y-P})
\begin{align*}
\beta^q\E[Y_t] &\gtrsim \beta^{q+1} \E|P|=
\beta^{q+1}|\ball(z, t)| \\
&\geq \beta^{q+1}|\ball(z, R_0)|.
\end{align*}
and conclude that inequality (b) holds.
\end{proof}

==> title/icml-title.tex <==

%%\icmltitle{$\alpha$-Correlation Clustering with $\ell_p$ Objective}
\icmltitle{Local Correlation Clustering with Asymmetric Classification Errors}


% It is OKAY to include author information, even for blind
% submissions: the style file will automatically remove it for you
% unless you've provided the [accepted] option to the icml2021
% package.

% List of affiliations: The first argument should be a (short)
% identifier you will use later to specify author affiliations
% Academic affiliations should list Department, University, City, Region, Country
% Industry affiliations should list Company, City, Region, Country

% You can specify symbols, otherwise they are numbered in order.
% Ideally, you should not use this facility. Affiliations will be numbered
% in order of appearance and this is the preferred way.
\icmlsetsymbol{equal}{*}

\begin{icmlauthorlist}
\icmlauthor{Jafar Jafarov}{equal,a}
\icmlauthor{Sanchit Kalhan}{equal,b}
\icmlauthor{Konstantin Makarychev}{equal,b}
\icmlauthor{Yury Makarychev}{equal,c}
\end{icmlauthorlist}
\icmlaffiliation{a}{University of Chicago, Chicago, IL, USA}
\icmlaffiliation{b}{Northwestern University, Evanston, IL, USA}
\icmlaffiliation{c}{TTIC, Chicago, IL, USA}
\icmlcorrespondingauthor{Jafar Jafarov}{jafarov@uchicago.edu}
\icmlcorrespondingauthor{Sanchit Kalhan}{skalhan@u.northwestern.edu}
% You may provide any keywords that you
% find helpful for describing your paper; these are used to populate
% the "keywords" metadata in the PDF but will not be shown in the document
\icmlkeywords{Machine Learning, ICML}
\vskip 0.3in


% this must go after the closing bracket ] following \twocolumn[ ...

% This command actually creates the footnote in the first column
% listing the affiliations and the copyright notice.
% The command takes one argument, which is text to display at the start of the footnote.
% The \icmlEqualContribution command is standard text for equal contribution.
% Remove it (just {}) if you do not need this facility.

%\printAffiliationsAndNotice{}  % leave blank if no need to mention equal contribution
\printAffiliationsAndNotice{\icmlEqualContribution} % otherwise use the standard text.

